Fairest Neighbors: Tradeoffs Between Metric Queries

Metric search commonly involves finding objects similar to a given sample object. We explore a generalization, where the desired result is a fair tradeoff between multiple query objects. This builds on previous results on complex queries, such as linear combinations. We instead use measures of inequality, like ordered weighted averages, and query existing index structures to find objects that minimize these. We compare our method empirically to linear scan and a post hoc combination of individual queries, and demonstrate a considerable speedup.

==> citecmds.tex <==
% Automatically generated from paper.bib by citegen.jl
% Include in document preamble witih \include{citecmds.tex}
% (Requires xparse.sty)
\ExplSyntaxOn
\makeatletter

\tl_new:N \l_citepref_tl

\def\@cite#1#2{[{\l_citepref_tl #1\if@tempswa ,~#2\fi}]}

\cs_new:Npn \__citeimpl:nnn #1 #2 #3 {
    \IfNoValueTF { #1 } {
        \cite{#3}
    } {
        \IfNoValueTF { #2 } {
            \cite[#1]{#3}
        } {
            \group_begin:
            \tl_set:Nn \l_citepref_tl { #1 ~ }
            \tl_if_empty:nTF { #2 } {
                \cite{#3}
            } {
               \cite[#2]{#3}
            }
            \group_end:
        }
    }
}

\DeclareDocumentCommand \citep { o o +m } {
    \__citeimpl:nnn {#1} {#2} {#3}
}

\NewDocumentCommand \citet { o o +m } {
    \tl_use:c { citeauthor_#3 }
    \nobreakspace
    \__citeimpl:nnn {#1} {#2} {#3}
}

\NewDocumentCommand \Citet { o o +m } {
    \tl_use:c { Citeauthor_#3 }
    \nobreakspace
    \__citeimpl:nnn {#1} {#2} {#3}
}

\NewDocumentCommand \citeauthor { m } {
    \tl_use:c { citeauthor_#1 }
}

\NewDocumentCommand \Citeauthor { m } {
    \tl_use:c { Citeauthor_#1 }
}

\NewDocumentCommand \citeyear { m } {
    \tl_use:c { citeyear_#1 }
}
\tl_set:cn{ citeauthor_Feustel:1982 } {
    Feustel~and~Shapiro
}

\tl_set:cn{ Citeauthor_Feustel:1982 } {
    Feustel~and~Shapiro
}

\tl_set:cn{ citeyear_Feustel:1982 } {
    1982
}

\tl_set:cn{ citeauthor_Zezula:2006 } {
    Zezula~et~al.
}

\tl_set:cn{ Citeauthor_Zezula:2006 } {
    Zezula~et~al.
}

\tl_set:cn{ citeyear_Zezula:2006 } {
    2006
}

\tl_set:cn{ citeauthor_Ciaccia:2000 } {
    Ciaccia~et~al.
}

\tl_set:cn{ Citeauthor_Ciaccia:2000 } {
    Ciaccia~et~al.
}

\tl_set:cn{ citeyear_Ciaccia:2000 } {
    2000
}

\tl_set:cn{ citeauthor_Yarygina:2011 } {
    Yarygina~et~al.
}

\tl_set:cn{ Citeauthor_Yarygina:2011 } {
    Yarygina~et~al.
}

\tl_set:cn{ citeyear_Yarygina:2011 } {
    2011
}

\tl_set:cn{ citeauthor_Ciaccia:1998 } {
    Ciaccia~et~al.
}

\tl_set:cn{ Citeauthor_Ciaccia:1998 } {
    Ciaccia~et~al.
}

\tl_set:cn{ citeyear_Ciaccia:1998 } {
    1998
}

\tl_set:cn{ citeauthor_Gonzales:2020 } {
    Gonzales~and~Perny
}

\tl_set:cn{ Citeauthor_Gonzales:2020 } {
    Gonzales~and~Perny
}

\tl_set:cn{ citeyear_Gonzales:2020 } {
    2020
}

\tl_set:cn{ citeauthor_Fagin:1999 } {
    Fagin
}

\tl_set:cn{ Citeauthor_Fagin:1999 } {
    Fagin
}

\tl_set:cn{ citeyear_Fagin:1999 } {
    1999
}

\tl_set:cn{ citeauthor_Chavez:2005 } {
    Ch{\'a}vez~and~Navarro
}

\tl_set:cn{ Citeauthor_Chavez:2005 } {
    Ch{\'a}vez~and~Navarro
}

\tl_set:cn{ citeyear_Chavez:2005 } {
    2005
}

\tl_set:cn{ citeauthor_Figueroa:2007 } {
    Figueroa~et~al.
}

\tl_set:cn{ Citeauthor_Figueroa:2007 } {
    Figueroa~et~al.
}

\tl_set:cn{ citeyear_Figueroa:2007 } {
    2007
}

\tl_set:cn{ citeauthor_Torra:1997 } {
    Torra
}

\tl_set:cn{ Citeauthor_Torra:1997 } {
    Torra
}

\tl_set:cn{ citeyear_Torra:1997 } {
    1997
}

\tl_set:cn{ citeauthor_Hetland:2019 } {
    Hetland
}

\tl_set:cn{ Citeauthor_Hetland:2019 } {
    Hetland
}

\tl_set:cn{ citeyear_Hetland:2019 } {
    2019
}

\tl_set:cn{ citeauthor_Moulin:2003 } {
    Moulin
}

\tl_set:cn{ Citeauthor_Moulin:2003 } {
    Moulin
}

\tl_set:cn{ citeyear_Moulin:2003 } {
    2003
}

\tl_set:cn{ citeauthor_Yianilos:1993 } {
    Yianilos
}

\tl_set:cn{ Citeauthor_Yianilos:1993 } {
    Yianilos
}

\tl_set:cn{ citeyear_Yianilos:1993 } {
    1993
}

\tl_set:cn{ citeauthor_Fredriksson:2007 } {
    Fredriksson
}

\tl_set:cn{ Citeauthor_Fredriksson:2007 } {
    Fredriksson
}

\tl_set:cn{ citeyear_Fredriksson:2007 } {
    2007
}

\tl_set:cn{ citeauthor_Tellez:2012 } {
    Tellez~and~Ch{\'a}vez
}

\tl_set:cn{ Citeauthor_Tellez:2012 } {
    Tellez~and~Ch{\'a}vez
}

\tl_set:cn{ citeyear_Tellez:2012 } {
    2012
}

\tl_set:cn{ citeauthor_Chen:2008 } {
    Chen~and~Lian
}

\tl_set:cn{ Citeauthor_Chen:2008 } {
    Chen~and~Lian
}

\tl_set:cn{ citeyear_Chen:2008 } {
    2008
}

\tl_set:cn{ citeauthor_Bustos:2006 } {
    Bustos~and~Skopal
}

\tl_set:cn{ Citeauthor_Bustos:2006 } {
    Bustos~and~Skopal
}

\tl_set:cn{ citeyear_Bustos:2006 } {
    2006
}

\makeatother
\ExplSyntaxOff


